APEx: Accuracy-Aware Differentially Private Data Exploration

Organizations are increasingly interested in allowing external data scientists to explore their sensitive datasets. Due to the popularity of differential privacy, data owners want the data exploration to ensure provable privacy guarantees. However, current systems for answering queries with differential privacy place an inordinate burden on the data analysts to understand differential privacy, manage their privacy budget, and even implement new algorithms for noisy query answering. Moreover, current systems do not provide any guarantees to the data analyst on the quality they care about, namely accuracy of query answers. We present APEx, a novel system that allows data analysts to pose adaptively chosen sequences of queries along with required accuracy bounds. By translating queries and accuracy bounds into differentially private algorithms with the least privacy loss, APEx returns query answers to the data analyst that meet the accuracy bounds, and proves to the data owner that the entire data exploration process is differentially private. Our comprehensive experimental study on real datasets demonstrates that APEx can answer a variety of queries accurately with moderate to small privacy loss, and can support data exploration for entity resolution with high accuracy under reasonable privacy settings.

==> overview.tex <==
%!TEX root=./main.tex
\subsection{Our Approach}\label{sec:overview}


We propose \system (Figure~\ref{fig:problemsetting}), an accuracy-aware privacy engine for sensitive data exploration. A data analyst can interact with the private data through \system using declaratively specified aggregate queries (Section~\ref{sec:explorequeries}). Our query language supports a large class of aggregates including linear counting queries (e.g., histograms and CDFs), iceberg queries (e.g., frequent patterns) and top-k queries, which are the building blocks of most data exploration workflows. \am{Cleaning ...}. Our language associates with each query an accuracy requirement (Section~\ref{sec:accuracy}). \system allows data analysts to pose an \textit{adaptively chosen} sequence of queries and accuracy requirements, i.e., the next query and its accuracy can depend on the previous queries.  


For each query in a sequence, \system employs an \textit{accuracy translator} that finds  a privacy level $\epsilon$ and a differentially private mechanism that answers the query while meeting the specified accuracy bound. Additionally, \system uses a \textit{privacy analyzer} to decide whether or not to answer a query such that the privacy loss to the analyst is always bounded by privacy budget $B$. We summarize the end-to-end \system in Section~\ref{sec:system-overview}, and decribe the accuracy translator and the privacy analysis in detail in Sections~\ref{sec:translation} and \ref{sec:analyzer}, respectively.




\input{queries}
\input{accuracy-measures}
\input{system-overview}




==> primitives.tex <==
\section{Privacy Primitives} \label{sec:primitives}

\subsection{Aggregate Primitives}
%consider all the leftside of the boolean predicate $\phi$  as a column of a table, e.g. similarity ...

{\bf Group By Queries with WHERE.}

\begin{lstlisting}
SELECT COUNT(*), A_i
    FROM D
    WHERE condition on A_j
    GROUP BY* A_i;
\end{lstlisting}

Discussion:
\begin{itemize}
\item $A_i$ and $A_j$ can be extended columns of table $D$. The query does not have to specify the Group by columns.
\item When the group by columns $A_i$ are not specified, this primitive is simply a linear counting query on the table $D$. The tolerance can be defined as
same as $(\alpha,\beta)$-\lc tolerance.
\item When the group by columns $A_i$ are specified, we will define mean square error for the histogram query.
\item The group by query is special here with * symbol, to denote we must specify the domain values for this group by column if it is unbounded.
The where condition can be one way to bound the domain range of the group by column, but more expressive ways should be included here.
\item COUNT(*) can be replaced by other aggregates, e.g. SUM, AVG, STD, COUNT DISTINCT, but their tolerance measures will be different.
\end{itemize}


{\bf Group By Queries with HAVING}
\begin{lstlisting}
SELECT A_i
    FROM D
    GROUP BY* A_i
    HAVING condition on COUNT(*);
\end{lstlisting}

Discussion:
\begin{itemize}
\item When the group by columns $A_i$ are not specified, this primitive is simply a linear counting query with conditions on the table $D$.
The tolerance can be defined as same as $(\alpha,\beta)$-\lcc tolerance.
\item When the group by columns $A_i$ are specified, the tolerance can be based on set difference.
\item Similar to the previous primitive, group by needs to be specially taken care.
\item COUNT(*) can be replaced by other aggregates, but tolerance measure will be different.
\end{itemize}


\subsection{Top-k Aggregate Primitives}

\begin{lstlisting}
SELECT COUNT(*) A_i
    FROM D
    GROUP BY* A_i
    ORDER BY COUNT(*) DESC;
\end{lstlisting}

Discussion:
\begin{itemize}
\item The group by columns $A_i$ must be specified, the tolerance can be the same as $(\alpha,\beta)$-\lct tolerance.
\item Similar to the previous primitive, group by needs to be specially taken care.
\item COUNT(*) can be replaced by other aggregates, but tolerance measure will be different.
\end{itemize}


\subsection{Other Primitives}
\begin{itemize}
\item Prefix cubes, blocked prefix cubes.
\item Select from a sample of D, rather than the entire dataset.
\item Linear regression
\end{itemize}

\eat{
This section formalizes the three types of aggregate query primitives supported in \system:
(i) linear counting queries,
(ii) linear counting queries with conditions, and
(iii) top-k linear counting queries.
We consider these primitives because:
(1) the definition of tolerance is different for these queries, and
(2) the differentially private algorithms that support these primitives are different.
\todo{(3) they can be used to express the aggregate queries commonly used in AQP (e.g. cite AQP++).}


\subsection{Linear Counting Query (\lc)}
There is much work on answering \emph{linear counting queries} under differential privacy \cite{Li:2010:OLC:1807085.1807104,Hay:2016:PED:2882903.2882931}.
An LC query on a table $D$, denoted by $q_{\phi}(\cdot)$,
returns the number of rows in the table that satisfy a boolean predicate $\phi:\rowdomain \rightarrow \{0,1\}$.
An LC query $q_{\phi}(D)$ can be expressed in SQL as
\begin{lstlisting}
SELECT COUNT(*) FROM $D$ WHERE $\phi$;
\end{lstlisting}

%Many cleaning tasks can be guided by this type of queries, such as identifying attributes with a small number of NULL values, or searching for effective transformations on attribute values to match records referring to the same entity.

Given an LC query $q$, we define the distance between the true output $q(D)$ and an approximate answer $a$ as the absolute difference $|q(D) - a|$. The error tolerance for a mechanism for answering an LC query is defined as:
\begin{definition}[$(\alpha,\beta)$-\lc tolerance]
Given a linear counting query $q_{\phi}$,
we say a mechanism $M:\tabledomain \rightarrow \mathbb{R}$
satisfies $(\alpha,\beta)$-\lc tolerance,
if for any table $D\in \tabledomain$,
\begin{eqnarray}
\Pr[|M(D) - q_{\phi}(D)| \geq \alpha] \leq \beta.
\end{eqnarray}
\end{definition}

\noindent LC queries can be used to guide several cleaning tasks.

\begin{example}[\lc Queries for NULLs]\label{eg:lc_missingvalue}
Counting the number of rows with NULL for an attribute is an \lc query on a base table $D$ which counts the number of rows in $D$ where the given attribute has `NULL' value. If the true answer is 10000, and the tolerance is $(\alpha = 10, \beta=.05)$, then the approximate answer should be within
$[9990,10010]$ with $95\%$ probability.
\end{example}

\noindent The \emph{sensitivity} of an LC query on a base table, or the max change in its output due to adding or removing a tuple in the input, is always $\leq 1$. LC queries can also be posed on views over the base table, and its sensitivity is bounded by the \emph{stability} of the view. Stability, defined as the number of tuples added or removed from a view due to adding or removing a single tuple in the base table, can be computed using well known methods \cite{McSherry:2009:PIQ:1559845.1559850, DBLP:journals/corr/JohnsonNS17}. In all our experiments, queries are either on base tables or views with stability 1; hence, \lc queries always have sensitivity 1.
\begin{example}[\lc Queries for Blocking]\label{eg:lc_blocking}
Given a dataset $D$, let $D_t$ be a training set that consists of pairs of records in $D$ and whether they are matching or non-matching records (as described in Sec.~\ref{sec:usecase_def}). Then, recall of the blocking predicate $P_b: cosine(2grams(r1.name),2grams(r2.name)) > 0.7$ can be computed by first answering a LC $q_{P_b}$ over the training set $D_t$ that counts the number of matching records, $D_t^+$, that satisfy the predicate $P_b$, and then dividing by the number of matching records in $D_t^+$, a known constant. Note that if each record in $D$ appears at most $m$ times in $D_t$, then the stability of $D_t$ (and the sensitivity of $q_{P_b}$) is at most $m$.
\end{example}


\subsection{\lc Query with Condition (\lcc)}
Given a table $D$, a linear counting with condition (\lcc) query $q_{\phi \theta c}$ returns a binary output ($\in \{0,1\}$) based on comparing an \lc query output $q_{\phi}(D)$ with a given threshold $c$. The comparison operator $\theta$ can be `$>,<,\geq,\leq$'.  The error tolerance for a mechanism answering an \lcc query $q_{\phi > c}$ is:
\begin{definition}[$(\alpha,\beta)$-\lcc tolerance]
A mechanism $M:\tabledomain \rightarrow \{\text{0,1}\}$
satisfies $(\alpha,\beta)$-\lcc tolerance for an \lcc query $q_{\phi,>c}$
if for any table $D$,
\begin{eqnarray}
\Pr[M(D) = \text{1} ~|~ q_{\phi}(D) < c-\alpha] \leq \beta \\
\Pr[M(D) = \text{0} ~|~ q_{\phi}(D) > c+\alpha] \leq \beta
\end{eqnarray}
\eat{
for $a=\text{True}$, we have
\begin{eqnarray}
q_{\phi}(D) \geq c-\alpha,
\end{eqnarray}
and for $a=\text{False}$, we have
\begin{equation}
q_{\phi}(D) \leq c + \alpha.
\end{equation}
}
\end{definition}
Error tolerance for other $q_{\phi \theta c}$ are defined analogously.

\begin{example}[\lcc Queries for NULLs]\label{eg:lcc_missingvalue}
Continuing with Example~\ref{eg:lc_missingvalue}, instead of querying for
the number of NULLs for an attribute, the cleaner can ask whether the number
of NULLs is greater than some threshold, say 1000.
Given a tolerance of $(\alpha = 10, \beta = .05)$,
then when the answer is $1$, with 95\% probability the true count is $> 1000-10$;
and when the answer is $0$, with 95\% probability the true count is $< 1000+10$;
\end{example}
Similarly, \lcc queries can be used to check if the quality of a blocking
scheme or a matching predicate reaches a threshold.
%The sensitivity of an LCC query on a table is always 1.


\subsection{\lc Top-K Query (\lct)}
Given a table $D$, a top-$k$ linear counting query
takes in a set of boolean formulae $\Phi=\{\phi_1,\ldots,\phi_L\}$,
and outputs the top-$k$ boolean formulae that are satisfied by
the largest (or the least) number of rows in the table,
 denoted by $q_{\phi_1,\ldots,\phi_L}^{k,\downarrow}$
(or  $q_{\phi_1,\ldots,\phi_L}^{k,\uparrow}$, respectively).
%We take the top-$k$ with largest values as an example and have
%the corresponding SQL form:
%\begin{lstlisting}
%SELECT p FROM
%   (SELECT $\phi_1$ p, COUNT(*) c FROM $D$ WHERE $\phi_1$
%    UNION  ...  UNION
%    SELECT $\phi_1$ p, COUNT(*) c FROM $D$ WHERE $\phi_l$)
%ORDER BY $c$ DSC LIMIT $k$;
%\end{lstlisting}
\begin{definition}[$(\alpha,\beta)$-\lct tolerance]
Given a top-$k$ linear counting query $q_{\phi_1,\ldots,\phi_L}^{k,\downarrow}$, we say that a mechanism $M:\tabledomain \rightarrow O$ with output $a=\{\phi_{i_1},\ldots, \phi_{i_k}\}$ satisfies $(\alpha,\beta)$-\lct tolerance if for any table $D\in \tabledomain$,
\begin{eqnarray}
\Pr[ |\{\phi \in M(D) ~|~ q_{\phi}(D) < c_k-\alpha \}| > 0] \leq \beta \\
\Pr[ |\{\phi \in (\Phi-M(D)) ~|~ q_{\phi}(D) > c_k + \alpha \}| = 0 ] \leq \beta
\end{eqnarray}
where $c_k$ is the answer to the $k^{th}$ largest \lc query.
\end{definition}
This definition is equivalent to saying that
with high probability
all boolean formulae $\phi$ in the output of the mechanism
have $q_{\phi}(D) > c_k-\alpha$,
and every $\phi\in \{\phi_1,\ldots,\phi_L\}$ with
$q_{\phi}(D) > c_k + \alpha$ is in the output.

\begin{example}[\lct Queries for Missing Values]\label{eg:lct_missingvalue}
Again continuing with Example~\ref{eg:lc_missingvalue}, suppose the cleaner
wants to prune out $k$ attributes with the most number of NULLs. Rather than using \lc queries counting the number of NULLs in each attribute, the cleaner could directly ask an \lct query.  For instance, suppose $\{A_1,A_2,\ldots,A_5\}$ have $\{10000,8000,200,100,50\}$ NULLs respectively.  The top $k=2$ attributes with the most number of missing values are $A_1,A_2$.
The number of NULLs in $A_2$, the $k$th largest \lc query answer, is 8000.
Given a tolerance of $(\alpha = 10, \beta = .05)$,
then with high probability, attributes selected in the output should have a true count larger than 8000-10, and attributes with true count larger than 8000+10 should be appear in the output.
\end{example}


}


==> ps.tex <==
%!TEX root=./main.tex
\section{Problem Definition \& Solution Overview}\label{sec:ps}

We aim to design a system that allows data analysts to explore a sensitive dataset $D$ held by a data owner by posing a sequence of declaratively specified queries that can capture typical data exploration workflows. Since the data are sensitive, the data owner would like the system provably bound the information disclosed about any one record in $D$ to the analyst. Since privacy preserving mechanisms introduce error, the data analyst must be able to specify accuracy bounds on each query. 


\noindent{\textbf{Problem:}}
Our goal is to design a system that can: 
\squishlist
\item Support a declaratively specified aggregate queries that capture a wide variety of data exploration tasks. 
\item Allow analysts to specify accuracy bounds on queries. 
\item Translate an analyst query into a differentially private mechanism with least privacy loss $\epsilon$ such that it can answer the query while meeting the accuracy bound.
\item Prove that for any sequence of queries, the analysts view of entire data exploration process satisfies $B$-differential privacy, where $B$ is a owner specified privacy budget. 
\squishend


\noindent{\textbf{Solution Overview:}}
We propose \system (Figure~\ref{fig:problemsetting}), an accuracy-aware privacy engine for sensitive data exploration. \system solves the aforementioned challenges as follows: 
\squishlist
\item A data analyst can interact with the private data through \system using declaratively specified aggregate queries. Our query language supports three types of aggregate queries: (i) \textit{workload counting queries} that capture the large class of linear counting queries (e.g., histograms and CDFs) which are a staple of statistical analysis, (ii) \textit{iceberg queries}, which capture HAVING queries in SQL and frequent pattern queries, and (iii) \textit{top-k queries}. These queries form the building blocks of several data exploration workflows. In Section~\ref{sec:casestudy}, we express two important data cleaning tasks, namely blocking and pair-wise matching, using sequences of queries from our language.
\item In our language each query is associated with intuitive accuracy bounds that permit \system to use differentially private mechanisms that introduce noise while meeting the accuracy bound. 
\item For each query in a sequence, \system employs an \textit{accuracy translator} that finds  a privacy level $\epsilon$ and a differentially private mechanism that answers the query while meeting the specified accuracy bound. For the same privacy level, the mechanism that answers a query with the least error differs depending on the query and dataset. Hence, \system implements a suite of differentially private mechanisms for each query type, and given an accuracy bound chooses the mechanism that incurs the least privacy loss based on the input query and dataset. 
\item \system uses a \textit{privacy analyzer} to decide whether or not to answer a query such that the privacy loss to the analyst is always bounded by a budget $B$. The privacy analysis is novel since the privacy loss of each mechanism is chosen based on the query's accuracy requirement, and since some mechanisms have a data dependent privacy loss.   
\squishend
We describe our query language in Section~\ref{sec:queries},  the end-to-end \system system in Section~\ref{sec:system-overview}, the accuracy translator in Section~\ref{sec:translation} and the privacy analysis in Section~\ref{sec:analyzer}.
 



 

==> rdp.tex <==
\newcommand{\order}{\lambda}

\subsection{R\'enyi Differential Privacy}\label{sec:rdp}

\begin{definition}[$(\order,\epsilon)$)-RDP~\cite{DBLP:journals/corr/Mironov17}]
A randomized mechanism $M:\tabledomain \rightarrow \mathcal{O}$
is said to have $\epsilon$-R\'enyi differential privacy of order $\order$,
or $(\order,\epsilon)$-RDP for short, if for any $D,D'\in \tabledomain$
that differ by adding or removing a record (i.e., $|D \setminus D' \cup D' \setminus D| = 1$),
we write $P$ and $Q$ for the distributions of $M(D)$ and $M(D')$,
it holds that
\begin{equation}
D_{\order}( P\|Q ))\leq \epsilon,
\end{equation}
where
$D_{\order}(P\|Q) = \frac{1}{\order -1}\log \mathbb{E}_{x\sim Q} ( \frac{P(x)}{Q(x)} )^{\order}$
for $\order >1$.
\end{definition}

When the order $\order$ goes to $\infty$, $(\order,\epsilon)$-RDP guarantee is equivalent to
$\epsilon$-DP.

\todo{Laplace mechanism $Lap(b)$} satisfies $(\order,\epsilon_{b}(\order))$-RDP, where
\[
    \epsilon_{b}(\order)=
\begin{cases}
\frac{1}{\order-1}\log \{\frac{\order e^{(\order-1)/b}}{2\order-1} + \frac{(\order-1)e^{-\order/b}}{2\order-1} \},&\text{if } \order >1 \\
1/b + e^{-1/b}-1, & \text{if } \order= 1\\
1/b,              & \text{if }\order \rightarrow \infty
\end{cases}
\]

\todo{Gaussian mechanism $G(\sigma)$} satisfies $(\order,\epsilon_{\sigma}(\order)$-RDP, where
\[
  \epsilon_{\sigma}(\order) = \order/\sigma^2
\]

\eat{
%change to proposition
\begin{theorem}[Adaptive Sequential Composition]
Suppose that a mechanism $\mathcal{M}$
consists of a sequence of adaptive mechanisms $M_1,\ldots,M_i$
where $M_l: \prod_{j=1}^{l-1} \mathcal{O}_j \times \tabledomain \rightarrow \mathcal{O}_l.$
For any order $\order >1$,
if $M_l$ satisfies $(\order,\epsilon_l)$-RDP for all $l\in \{1,\cdots,i\}$,
then mechanism $\mathcal{M}$ satisfies $(\order,\sum_{j=1}^i \epsilon_j)$-RDP.
\end{theorem}


Consider a mechanism $\mathcal{M}$
consists of a sequence of adaptive Laplace mechanisms $Lap(b_1),\ldots,Lap(b_i)$,
then $\mathcal{M}$ satisfies $(\order,\epsilon_{b_1,\ldots,b_i}(\order))$-RDP, where
\[
    \epsilon_{b_1,\ldots,b_i}(\order)=
\begin{cases}
\sum_{j=1}^i \frac{1}{\order-1}\log \{\frac{\order e^{(\order-1)/b_j}}{2\order-1} + \frac{(\order-1)e^{-\order/b_j}}{2\order-1} \},&\text{if } \order >1 \\
\sum_{j=1}^i 1/b_j + e^{-1/b_j}-1, & \text{if } \order= 1\\
\sum_{j=1}^i 1/b_j,              & \text{if }\order \rightarrow \infty
\end{cases}
\]

If $b_1,b_2,\ldots,b_i$ are all the same value, let's say $b$, then
\[
    \epsilon_{b_1,\ldots,b_i}(\order)=
\begin{cases}
\frac{i}{\order-1}\log \{\frac{\order e^{(\order-1)/b}}{2\order-1} + \frac{(\order-1)e^{-\order/b}}{2\order-1} \},&\text{if } \order >1 \\
i\cdot ( 1/b + e^{-1/b}-1), & \text{if } \order= 1\\
i/b,              & \text{if }\order \rightarrow \infty
\end{cases}
\]
}


\begin{theorem}[Adaptive Sequential Composition \cite{DBLP:journals/corr/Mironov17}]
Let mechanism $M_1:\tabledomain \rightarrow \mathcal{O}_1$ be $(\order,\epsilon_1)$-RDP and
$M_2:\mathcal{O}_1 \times \tabledomain \rightarrow \mathcal{O}_2$ be $(\order,\epsilon_2)$-RDP,
then mechanism defined as $(X,Y)$, where $X\sim M_1(D)$ and $Y\sim M_2(X,D)$, satisfies $(\order, \epsilon_1+\epsilon_2)$-RDP.
\end{theorem}



\eat{
%change to proposition
\begin{theorem}[From RDP to $(\epsilon,\delta)$-DP~\cite{DBLP:journals/corr/Mironov17}] If $M$ is an $(\order,\epsilon)$-RDP mechanism,
it also satisfies $(\epsilon+\frac{\log(1/\delta)}{\order-1},\delta)$-differential privacy for any $0<\delta<1$.
\end{theorem}

\todo{Given $(B,\delta)$-DP, we can determine the privacy cost $B(\order)$ under RDP at each order $\order$,
where $B(\order)= B-\frac{\log(1/\delta)}{\order-1}$. [not necessarily true]}
}

\subsubsection{Overall Privacy Guarantee}

We show the following guarantee: any sequence of interactions between cleaning engineer and \system satisfies $(\order,B)$-RDP, where $B$ is the privacy budget specified by the data owner.
In order to state this guarantee formally, we first need the notion of a \emph{transcript of interaction} between \system and the cleaning engineer.

We define the transcript of interaction $\trans$ as an alternating sequence of queries (with tolerances) posed to \system and answers returned by \system. $\trans$ encodes the cleaner's view of the private database. More formally,
\begin{itemize}
	\item The transcript $\trans_i$ after $i$ interactions is a sequence $[(q_1, \alpha_1, \beta_1), (\omega_1, \epsilon_1), \ldots, (q_i, \alpha_i, \beta_i), (\omega_i, \epsilon_i)]$, where $(q_i, \alpha_i, \beta_i)$ are queries with tolerances, and $\omega_i$ is the answer returned by \system and $\epsilon_i$ the actual privacy loss associated with that answer at given order $\order$.
	\item Given $\trans_{i-1}$ the cleaner chooses the next query $(q_{i+1}, \alpha_{i+1}, \beta_{i+1})$ adaptively. We model this using a (possibly randomized) algorithm $\mathbb{C}$ that maps a transcript $\trans_{i-1}$ to $(q_i, \alpha_i, \beta_i)$; i.e., $\mathbb{C}(\trans_{i-1}) = (q_i, \alpha_i, \beta_i)$. Note that the cleaner algorithm $\mathbb{C}$ does not access the private database.
	\item Given a query with tolerance $(q_i, \alpha_i, \beta_i)$, \system translates it to a mechanism $M_i$ with a maximum privacy loss of $\epsmax_i$. While  $M_i$ itself is randomized, the translation between $(q_i, \alpha_i, \beta_i)$ and $M_i$ is deterministic and independent of the private database.
          \item \system decides whether to run the mechanism $M_i$ based on $\epsmax_i$ and $\trans_{i-1}$ (deterministic and independent of the private database too); and then runs this mechanism if it decides so. Hence, the output of this process is a pair $(\omega_i, \epsilon_i)$ and we denote this process $M^+_i$. The actual output $\omega_i$ is either a value in the range of $M_i$ or $\bot$, which denotes that the query was \emph{declined} by \system. $\epsilon_i$ is the \emph{actual} privacy loss due to running $M_i$. If the output is $\bot$, then $\epsilon_i = 0$, since the mechanism was not executed. When the query is not declined by \system, for mechanisms described in Section~\ref{sec:ind_tran} (i.e., LM, LCM, LTM), the actual privacy loss is always equal to the maximum privacy loss, i.e., $\epsilon_i = \epsmax_i$. For LCMP and LCMMP, the actual privacy loss can be smaller; i.e. $\epsilon_i \leq \epsmax_i$.
          %\item We assume that the output of every mechanism $M_i$ on private database $D$ is a pair $(\omega_i, \epsilon_i)$. The actual output $\omega_i$ is either a value in the range of $M_i$ or $\bot$, which denotes that the query was \emph{declined} by \system. $\epsilon_i$ is the \emph{actual} privacy loss due to running $M_i$. If the output is $\bot$, then $\epsilon_i = 0$, since the mechanism was not executed. When the query is not declined by \system, for mechanisms described in Section~\ref{sec:ind_tran} (i.e., LM, LCM, LTM), the actual privacy loss is always equal to the maximum privacy loss, i.e., $\epsilon_i = \epsmax_i$. For LCMP and LCMMP, the actual privacy loss can be smaller; i.e. $\epsilon_i \leq \epsmax_i$.
	\item Let $Pr[\trans_i| D]$ denote the probability that the transcript of interaction is $\trans_i$ given that the input database is $D$. The probability is over the randomness in the cleaners choices $\mathbb{C}$ and the randomness in the mechanisms $M_1, \ldots, M_i$ executed by \system.
\end{itemize}


Similarly, we can define valid transcripts for RDP.

\begin{definition}[Valid Transcripts]
  A transcript of interaction $\trans_i$ is a \emph{valid}  transcript if given a privacy budget $B$ the following conditions hold:
	\begin{itemize}
		\item $B(\trans_{i-1}) = \sum_{j = 1}^{i-1} \epsilon_j \leq B$, and
		\item Either $B(\trans_{i-1}) + \epsmax_i \leq B $, or $\omega_i = \bot$.
	\end{itemize}
\end{definition}

We are now ready to state the privacy guarantee:

\begin{theorem}[\system Privacy Guarantee]\label{thm:rdp_privacy}
Given a privacy budget $B$ for RDP at order $\order$,
the following are true:
\begin{enumerate}
\item for all $i>0$, all the transcripts $\trans_i$ generated by \system are valid;
\item for any pair of databases $D$, $D'$ that differ in one row (i.e., $|D \setminus D' \cup D' \setminus D| = 1$), for all $i>0$,
let $P_i$ and $Q_i$ be the distributions over \system transcripts generated from $D$ and $D'$ respectively after $i$ interactions,
\begin{equation}
D_{\order}(P_i \| Q_i) \leq B.
\end{equation}
\end{enumerate}
\end{theorem}
\begin{proof}
(1) directly follows from the definition of a valid transcript and these are the only kinds of transcripts a cleaner sees when interacting with \system.

(2) can be shown as follows using induction.

\noindent{\underline{Base Case:}} When the transcript is empty, it is clear that $D_{\order}(P_0 \|Q_0) = 0\leq B$.

\noindent{\underline{Induction step:}}
For $i>0$, let $\trans_i = \trans_{i-1} || [(q_i, \alpha_i, \beta_i), (\omega_i, \epsilon_i)]$ be a valid \system transcript of length $i$.
%Note that it is a deterministic mapping from $(q_i,\alpha_i,\beta_i)$ to $M_i^+$, we have
Here we consider $\epsilon_i$ is adaptively chosen based on $\trans_{i-1}$, and hence we have

\begin{eqnarray}
&&P_i(\trans_i) = \Pr[\trans_i|D] \\
&=& \Pr[\trans_{i-1}|D] \Pr[(\epsilon_i)|\trans_{i-1}] \Pr[\omega_i|D,\epsilon_{i}] \nonumber
\end{eqnarray}

\begin{eqnarray}
&&Q_i(\trans_i) = \Pr[\trans_i|D'] \\
&=& \Pr[\trans_{i-1}|D'] \Pr[(\epsilon_i)|\trans_{i-1}] \Pr[\omega_i|D',\epsilon_{i}] \nonumber
\end{eqnarray}

Then we can show that
\begin{eqnarray}
&& e^{(\order-1)D_{\order}(P_{i+1}\|Q_{i+1})} = \mathbb{E}_{\trans_{i+1} \sim Q_{i+1}} (P_{i+1}(\trans_{i+1})/Q_{i+1}(\trans_{i+1}))^{\order} \nonumber\\
&=& \sum_{\trans_{i+1}} P_{i+1}(\trans_{i+1})^{\order} Q_{i+1}(\trans_{i+1})^{1-\order} \nonumber \\
&=& \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot \sum_{\epsilon_{i+1}}\big\{ \Pr[\epsilon_{i+1}|\trans_i] \cdot \nonumber \\
&& \sum_{\omega_{i+1}} \Pr[\omega_{i+1}|D,\epsilon_{i+1}]^{\order} \Pr[\omega_{i+1}|D',\epsilon_{i+1}]^{1-\order} \big\} \Big\} \nonumber \\
&\leq & \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot \sum_{\epsilon_{i+1}} \big\{ \Pr[\epsilon_{i+1}|\trans_i] \cdot  \nonumber\\
&& e^{(\order-1)(\epsilon_{i+1})} \big\} \Big\} \nonumber \\
&\leq & \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot \sum_{\epsilon_{i+1}} \big\{ \Pr[\epsilon_{i+1}|\trans_i] \cdot \nonumber\\
&& e^{(\order-1)(B-B(\trans_i))} \big \} \Big\} \nonumber \\
&\leq & \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot e^{(\order-1)(B-B(\trans_i))} \Big\} \nonumber \\
&\leq & \sum_{\trans_{i-1}} \Big\{\Pr[\trans_{i-1}|D]^{\order}\Pr[\trans_{i-1}|D']^{1-\order}  e^{(\order-1)(B-B(\trans_{i-1}))} \cdot \nonumber \\
&& \sum_{\epsilon_i} \big\{ \Pr[\epsilon_i|\trans_{i-1})] e^{(1-\order)\epsilon_i}
\sum_{\omega_{i}} \Pr[\omega_{i}|D,\epsilon_i]^{\order} \Pr[\omega_{i}|D',\epsilon_i]^{1-\order}  \big\} \Big\} \nonumber \\
&\leq & \sum_{\trans_{i-1}} \Big\{\Pr[\trans_{i-1}|D]^{\order}\Pr[\trans_{i-1}|D']^{1-\order}  e^{(\order-1)(B-B(\trans_{i-1}))} \cdot \nonumber \\
&& \sum_{\epsilon_i} \big\{ \Pr[\epsilon_i|\trans_{i-1})] e^{(1-\order)\epsilon_i} e^{(\order-1)\epsilon_i}  \big\} \Big\} \nonumber \\
&\leq & \sum_{\trans_{i-1}} \Big\{\Pr[\trans_{i-1}|D]^{\order}\Pr[\trans_{i-1}|D']^{1-\order} \cdot e^{(\order-1)(B-B(\trans_{i-1}))} \Big\} \nonumber \\
&\leq & .... \nonumber \\
&\leq & e^{(\order-1)(B-B(\trans_0))} = e^{(\order-1)B}
\end{eqnarray}
\end{proof}

\eat{
\begin{eqnarray}
&&P_i(\trans_i) = \Pr[\trans_i|D] \\
&=& \Pr[\trans_{i-1}|D] \Pr[(q_i,\alpha_i,\beta_i)|\trans_{i-1}] \Pr[\omega_i,\epsilon_i|D] \nonumber
\end{eqnarray}

\begin{eqnarray}
&&Q_i(\trans_i) = \Pr[\trans_i|D'] \\
&=& \Pr[\trans_{i-1}|D'] \Pr[(q_i,\alpha_i,\beta_i)|\trans_{i-1}] \Pr[\omega_i,\epsilon_i|D'] \nonumber
\end{eqnarray}

Then we can show that
\begin{eqnarray}
&& \exp((\order-1)D_{\order}(P_{i+1}\|Q_{i+1})) \nonumber\\
&=& \mathbb{E}_{\trans_{i+1} \sim Q_{i+1}} (P_{i+1}(\trans_{i+1})/Q_{i+1}(\trans_{i+1}))^{\order} \nonumber\\
&=& \sum_{\trans_{i+1}} P_{i+1}(\trans_{i+1})^{\order} Q_{i+1}(\trans_{i+1})^{1-\order} \nonumber \\
&=& \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot \nonumber \\
&& \sum_{(q_{i+1},\alpha_{i+1},\beta_{i+1})} \Pr[(q_{i+1},\alpha_{i+1},\beta_{i+1}|\trans_i] \cdot \nonumber \\
&& \sum_{(\omega_{i+1},\epsilon_{i+1})} \Pr[(\omega_{i+1},\epsilon_{i+1})|D]^{\order} \Pr[(\omega_{i+1},\epsilon_{i+1})|D']^{1-\order} \Big\} \nonumber \\
&\leq & \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot \nonumber \\
&& \sum_{(q_{i+1},\alpha_{i+1},\beta_{i+1})} \Pr[(q_{i+1},\alpha_{i+1},\beta_{i+1}|\trans_i] \cdot \nonumber\\
&& \cdot\exp((\order-1)(B-B(\trans_i))) \Big\} \nonumber \\
&\leq & \sum_{\trans_i} \Big\{\Pr[\trans_i|D]^{\order}\Pr[\trans_i|D']^{1-\order} \cdot \exp((\order-1)(B-B(\trans_i))) \Big\} \nonumber \\
&\leq & \sum_{\trans_{i-1}} \Big\{\Pr[\trans_{i-1}|D]^{\order}\Pr[\trans_{i-1}|D']^{1-\order} \cdot \nonumber \\
&& \exp((\order-1)(B-B(\trans_{i-1}))) \cdot \sum_{(q_i,\alpha_i,\beta_i)} \Pr[(q_i,\alpha_i,\beta_i|\trans_{i-1})] \cdot \nonumber\\
&& \sum_{(\omega_{i},\epsilon_{i})} \Pr[(\omega_{i},\epsilon_{i})|D]^{\order} \Pr[(\omega_{i},\epsilon_{i})|D']^{1-\order}  \cdot \exp((\order-1)(-\epsilon_i)) \Big\} \nonumber \\
&\leq & \sum_{\trans_{i-1}} \Big\{\Pr[\trans_{i-1}|D]^{\order}\Pr[\trans_{i-1}|D']^{1-\order} \cdot\exp((\order-1)(B-B(\trans_{i-1}))) \cdot \nonumber \\
&& \sum_{(q_i,\alpha_i,\beta_i)} \Pr[(q_i,\alpha_i,\beta_i|\trans_{i-1})] \Big\} \nonumber \\
&\leq & \sum_{\trans_{i-1}} \Big\{\Pr[\trans_{i-1}|D]^{\order}\Pr[\trans_{i-1}|D']^{1-\order} \cdot\exp((\order-1)(B-B(\trans_{i-1}))) \nonumber \\
&\leq & .... \nonumber \\
&\leq & \exp((\order-1)(B-B(\trans_0))) = \exp((\order-1)B)
\end{eqnarray}
\end{proof}
}


\todo{Moment Accountant Method.}
At iteration $i$, consider $\order^* = argmin_{\order} B_i(\order) + \frac{\log(1/\delta)}{\order-1}$, which corresponds to $(\epsilon_i,\delta)$-DP,
where $\epsilon_i = B_i(\order^*) + \frac{\log(1/\delta)}{\order^*-1} \leq B_g$.
At this $\order^*$, for iterations $j<i$, we have
\begin{eqnarray}
\epsilon_j &=& B_j(\order^*) + \frac{\log(1/\delta)}{\order^*-1} \leq  B_i(\order^*) + \frac{\log(1/\delta)}{\order^*-1} \leq  B_g \nonumber
\end{eqnarray}



\subsection{Guassian Mechanism based Translation.}

Similar to the definition of Laplace Mechanism, we first formally define Guassian Mechanism.

\begin{definition}[Gaussian Mechanism]
Let function $f$ be a composite of $d$ \lc queries $\{q_1, ..., q_d\}$ releasing $d$ values: $f: D \rightarrow R^d$. Let $\mathcal{N}(\mu, \sigma^2)$ represent a Gaussian distribution with mean $=\mu$ and variation $=\sigma^2$.
The Gaussian Mechanism for $f$ is defined as:
$GM_{\sigma, f}(D) = \{q_i(D) + \mathcal{N}(0, \sigma^2)\}, \forall q_i \in f$.
\end{definition}

Under GM, we can translate a $(\alpha, \beta)-\lc$ tolerance to $(\lambda, \epsilon)$-RDP cost with the following theorem: 

\begin{theorem}
The  $(\alpha, \beta)-\lc$ tolerance is achievable on Gaussian Mechanism, denoted by $GM_{\sigma, f}^{\alpha,\beta}(D)$ i.e.
$\forall i\in \{1,...d\}, \Pr[|GM_{\sigma, f_d}^{\alpha,\beta}.q_i(D) - q_{i}(D)| \geq \alpha] \leq \beta$, with the the $(\lambda, \epsilon)$-Renyi differential privacy cost of $\epsilon=\frac{\lambda d}{2\sigma^2}$.

\end{theorem}

By definition of $(\alpha, \beta)$-tolerance, we can find the parameter $\sigma$ by the calculating inverse cumulative probability of the standard Guassian distribution with probability $p=\beta /2$. \system follows the similar translation patterns in Section~\ref{sec:ind_tran} for other query types, except using GM, as demonstrated above for the \lc query. In the rest of experiments, we will focus on \lc query to compare different mechanisms (Section~\ref{exp:diff_mechanisms}) and different privacy analyzers (Section~\ref{exp:diff_analyzers}).


==> recommend.tex <==
\section{Recommender}\label{sec:recommend}


==> usecase_er.tex <==
%!TEX root=./main.tex
\section{Case Study II: Entity Resolution}
Entity Resolution (ER) is an important data cleaning process which discovers the duplicate records that refer to the same entity. In general, the ER process can be organized into two tasks: 1) Block Task, where the goal is an efficient blocking function to keep high recall while prune unnecessary comparisons, since the quadratic number $O(n^2)$ of comparisons makes ER unpractical even when the number of record $n$ is moderate. 2) Matching Task, in which the cleaning engineer aims to find effective matching functions to figure out real duplicated records with reasonable number of the comparisons. A data cleaning engineer usually requires to interact and explore data in order to form correct ER functions. As observed in previous studies~\cite{DBLP:conf/amw/CarvalhoLM15}, the interaction can be implemented by asking aggregate queries. 
In this case study, we demonstrate that privacy-preserving entity resolution is possible with our private data exploration primitives, and show how this can be achieved by both the real and synthetic cleaning engineers.

In this case study, we use $D=$ {\tt citations}~\cite{magellandata} data, which include publication records of $2616$ and $64263$ from two bibliography sources of DBLP and Google Scholar, respectively. Each record has $4$ common attributes, and records from two sources may refer to the same publication. We sample $r_1$ from DBLP and $r_2$ from Google Scholar to form a set of record pairs $D_t=\{(r_1, r_2)\}$ where each pair has a label either true duplicate or false. The truth of the record pair is given from the data set, and we choose to make half of record pairs as duplicates. During the record pair construction, we ensure that any record can appear at most once. We use two sets of $D_t$ of different sizes, where $|D_{t1}|=1000$ and $|D_{t2}|=4000$.

  
\subsection{ER by Human Cleaning Engineers}
We conducted a user study\footnote{This test has been reviewed and received ethics clearance
through a University of Waterloo Research Ethics Committee (ORE$\#22665$).} at the University of Waterloo to ask data cleaning experts to complete an entity resolution task by using the data exploration primitives proposed in this paper. $8$ users were recruited and each was asked to complete one matching task and one blocking task on $D_{t1}$ at a given and fixed tolerance $\alpha = t|D_{t1}|$, where $t \in \{0, 0.02, 0.08, 0.32\}$. The matching task and blocking task were conducted and measured independently.

With the set of primitive templates provided by \system, the user issued a sequence of primitive queries. The \system answered one query at a time within the given query tolerance and sent the answer back to the user. The user refined the ER functions gradually and chose what query to ask next, or terminated. In these tests, users had no privacy constraint $B=\infty$, and hence they could ask unlimited number of queries until they were satisfied with the results.

After analyzing the user issued queries, we found out that most of the queries were WCQ measuring the quality of blocking or matching predicates. An example of such queries is the following:
\begin{lstlisting}[mathescape=true]
BIN $D_{t1}$ ON COUNT(*)
WHERE $W=\{$
      $cosine(2gram(r_1.ttl), 2gram(r_2.ttl)) > 0.9 \wedge l=true$,
      $cosine(2gram(r_1.ttl), 2gram(r_2.ttl)) > 0.8 \wedge l=true$,
      $\ldots$
      $cosine(2gram(r_1.ttl), 2gram(r_2.ttl)) > 0.5 \wedge l=true\}$
ERROR $20$ CONFIDENCE $0.9995$;
\end{lstlisting}
The above query measures how many true duplicates that using cosine similarity function over the $2gram$ of title at different thresholds can catch, whereas the probability that noisy counting deviates less than $20$ is $0.9995$. The answer provided the users insights on the data (e.g., the usefulness of attribute title) and on the predicates. Through the accumulated knowledge, the user eventually came up with a blocking/matching function.

\begin{figure*}[h]
	\centering
	%\begin{subfigure}[h]{0.25\textwidth}%
	%	\includegraphics[width=\textwidth]{../../figure/experiments/quality_np_random}%
	%	\caption{Arbitrary robot cleaners}
	%	\label{fig:intro_quality_np_random}
	%\end{subfigure}%}
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/quality_np}%
		\caption{Good cleaners (no noise)}
		\label{fig:intro_quality_np}
	\end{subfigure}%
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/quality_tolerance_BS}%
		\caption{Blocking with tolerance}
		\label{fig:intro_blocking_quality_tolerance}
	\end{subfigure}%
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/quality_tolerance_MS}%
		\caption{Matching with tolerance}
		\label{fig:intro_matching_quality_tolerance}
	\end{subfigure}%
	\caption{ Cleaning quality on blocking and matching tasks on {\tt citations} dataset:
                %(a) shows that self-tuned tools represented by arbitrary robot cleaners are limited;
                (a) shows that good cleaners (including human and manually designed robots) achieve high quality using true aggregate statistics;
		(b) and (c) show that the cleaning quality using noisy aggregate statistics decreases as noise level (tolerance) increases.}\label{fig:intro}
\end{figure*}

We use \emph{recall} and \emph{F1} score to measure the end to end cleaning quality of blocking and matching results. Figure~\ref{fig:intro} shows the users' qualities under different settings (red points). Figure~\ref{fig:intro_quality_np} shows that without noise (when $ERROR=0$) added to the answers, the users can achieve very good ER results. Figures~\ref{fig:intro_blocking_quality_tolerance} and ~\ref{fig:intro_matching_quality_tolerance} together show that when small noise was added, the users were still able to achieve good recall and F1, but the quality score decreased as tolerances went large. This is expected because larger error misled users' decision. The results implies that the primitives are useful to complete an ER task.


\subsection{ER by Robot Cleaning Engineers}
This section describes the program simulating human cleaning engineers (called robot cleaners). Robot cleaners are desirable to scale out for helping further to investigate the relations of many aspects of the primitives such as the effects of privacy constraint and error tolerance. We first describe how we generate human-alike robot cleaners to prove the effectiveness of robot cleaners.

Through analyzing the behavior of real users in the user test, we observed two type of actions that users incurred:\\
\noindent
\underline{Type-I: Queries with Tolerance.}
This type of actions basically issues queries using the primitives. This typically includes profiling the data (e.g., query distribution of an attribute using WCQ primitives), and quantify the quality of predicates. The following query is of WCQ type to profile empty attributes:
\begin{lstlisting}[mathescape=true]
BIN $D_{t1}$ ON COUNT(*)
WHERE $W=\{ttl \ is \ NULL, ttl \ is \ NULL, vn \ is \ NULL, year \ is \ NULL \}$
ERROR $\alpha$ CONFIDENCE $1-\beta$;
\end{lstlisting}

The corresponding TCQ query to select the top-$2$ attributes with least NULLs is represented as:
\begin{lstlisting}[mathescape=true]
BIN $D_{t1}$ ON COUNT(*)
WHERE $W=\{ttl \ is \ NULL, ttl \ is \ NULL, vn \ is \ NULL, year \ is \ NULL \}$
ORDER BY COUNT() DESC LIMIT 2
ERROR $\alpha$ CONFIDENCE $1-\beta$;
\end{lstlisting}

Type-I queries can be more powerful to evaluate predicates. The following query is to measure the effectiveness of Jaccard similarity over attribute authors, at a presence of a given predicate.
\begin{lstlisting}[mathescape=true]
BIN $D_{t1}$ ON COUNT(*)
WHERE $W=\{$
    $l=true \wedge cosine(2grams(r_1.ttl),2grams(r_2.ttl)) \le 0.6$
          $\wedge jaccard(ST(r_1.thr), ST(r_2.thr)) > 0.9,$
    $l=true \wedge cosine(2grams(r_1.ttl),2grams(r_2.ttl)) \le 0.6$
          $\wedge jaccard(ST(r_1.thr), ST(r_2.thr)) > 0.8,$
    $l=true \wedge cosine(2grams(r_1.ttl),2grams(r_2.ttl)) \le 0.6$
          $\wedge jaccard(ST(r_1.thr), ST(r_2.thr)) > 0.7 \}$
ERROR $\alpha$ CONFIDENCE $1-\beta$;
\end{lstlisting}

The ICQ version of above query is to include the $HAVING$ to return the predicates only:
\begin{lstlisting}[mathescape=true]
BIN $D_{t1}$ ON COUNT(*)
WHERE $W=\{$
    $l=true \wedge cosine(2grams(r_1.ttl),2grams(r_2.ttl)) \le 0.6$
          $\wedge jaccard(ST(r_1.thr), ST(r_2.thr)) > 0.9,$
    $l=true \wedge cosine(2grams(r_1.ttl),2grams(r_2.ttl)) \le 0.6$
          $\wedge jaccard(ST(r_1.thr), ST(r_2.thr)) > 0.8,$
    $l=true \wedge cosine(2grams(r_1.ttl),2grams(r_2.ttl)) \le 0.6$
          $\wedge jaccard(ST(r_1.thr), ST(r_2.thr)) > 0.7 \}$
HAVING COUNT(*) > 100
ERROR $\alpha$ CONFIDENCE $1-\beta$;
\end{lstlisting}

We summarized all the predicates and found the parameter space of Type-I queries. Two class of robots were created: robots issue Type-I queries using WCQ only primitive, and robots issues Type-I queries using ICQ and TCQ primitives. 

\noindent
\underline{Type-II: Smart Cleaning Choices.}
This type of actions are the smart choices made by the cleaning engineer based on the knowledge of the engineer (including the sequence query answers learned so far in addition to the initial expertise and the preference of this engineer). Different cleaning engineers normally choose different sets/orders/criterion. Since Type-II action does not directly rely on the exploratory primitives, so we programmed the cleaning choices to always make decisions for high recall and F1 within a given blocking cost boundary.

By interleaving Type-I and Type-II actions, we formalized the cleaning strategies for blocking and matching. The detailed parameters are described in Appendix~\ref{sec:cleaner_model}. Figure~\ref{fig:intro} shows the quality of $100$ random generated robot cleaners (blue points) compared with human cleaners (red points). The robot cleaners can achieve similar results with human under all settings using our primitives. Therefore, we will use the robot cleaners to showcase the behavior of private data exploration for entity resolution.


\subsection{Evaluations on Private ER}

\subsubsection{Queries With No Privacy Constraint}

\subsubsection{Varying Privacy Constraint}

\subsubsection{Varying Tolerance}



==> usecase_ve.tex <==
%!TEX root=./main.tex
\section{Case Study I: Visual Exploration}
\label{sec:cs_ve}

\todo{benchmark description}

In this case study, the analyst wants to explore the data to learn the dominating factors that affect income. Piror work on interactive data exploration~\cite{DBLP:conf/sigmod/CrottyGZBK16} identified a sequence of $16$ queries on $D=$ {\tt census}~\cite{Dua:2017} dataset to model how an analyst would explore the data gradually, and follow-up work on approximate query processing~\cite{DBLP:journals/pvldb/GalakatosCZBK17} showed this visual exploration can be completed with approximate queries. In this case study, the original queries are benchmarked into two groups: histogram and prefix queries. Both the two groups can be fully expressed using the private primitives. For example, a $1$-D histogram template on {\tt sex} attribute can be expressed as follows:
\begin{lstlisting}[mathescape=true]
BIN Census ON COUNT(*)
WHERE $W=\{sex='Male', sex='Female' \}$
ERROR $\alpha$ CONFIDENCE $1-\beta$;
\end{lstlisting}


\eat{
\begin{lstlisting}[mathescape=true]
BIN Census ON COUNT(*)
WHERE $W=\{$
    $sex<>'Female' \wedge salary=0,$
    $sex<>'Female' \wedge salary<10000,$
    $sex<>'Female' \wedge salary<20000,$
    $\ldots$
    $sex<>'Female' \wedge salary < 100000\}$
ERROR $\alpha$ CONFIDENCE $1-\beta$;
\end{lstlisting}
}

After removing duplicated queries from the user study, the benchmark consists of $15$ one dimensional histogram queries, $8$ one dimensional prefix queries, and $2$ two dimensional histogram queries. The queries were derived from the past study~\cite{DBLP:journals/pvldb/GalakatosCZBK17}, and are numbered accordingly to represent their originality with previous work.

\eat{
\subsection{From Confidence Interval to $(\alpha,\beta)$-accuracy}
In approximate query processing, along with an approximated answer of a query $q$, AQP often returns a confidence interval $ci=(\theta, \phi)$ to quantity the estimation uncertainty. The confidence interval is an interval estimate of the true value. For example, a $(100,95\%)$ confidence interval of a query answer $q \pm 100$ means there is $95\%$ probability that the true answer is within this range. The notation of confidence interval perfectly aligns with the $(\alpha,\beta)$-accuracy that is used in our query primitives if $q$ is a counting query, as $\alpha$ is equivalent to $\theta$ and $\beta = 1 - \phi$. By this way, we can use the private primitives to seamlessly satisfy AQP requirements while additionally quantifying the privacy cost. 
}

\subsection{Evaluations}
All the results are based on $100$ repeated runs over $|D|=32561$ records


\subsubsection{Effectiveness of Translator}

For effectiveness, there are two aspects: accuracy and privacy. For accuracy, given a workload query consisting of $L$ predicates, WCQ returns $L$ noisy counts, and hence the accuracy can be measured by the empirically maximum error that was introduced into any predicate. ICQ bi-classifies the predicates with respect to the condition $c$, and thus the accuracy can be measured by the correctness ratio of the classification. TCQ outputs the top $k$ predicates and its accuracy is represented by recall of the true top $k$ predicates.

\eat{
\begin{figure*}[h]
	\centering
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/census_accuracy_1d_hist_wcq}%
		\caption{1-D Histogram Queries}
		\label{fig:}
	\end{subfigure}%
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/census_accuracy_1d_prefix_wcq}%
		\caption{1-D Prefix Queries}
		\label{fig:}
	\end{subfigure}%
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/census_accuracy_2d_hist_wcq}%
		\caption{2-D Histogram Queries}
		\label{fig:}
	\end{subfigure}%
	\caption{Accuracy of $(0.0032|D|, 0.0005)$-accuracy WCQ using Laplace Mechanism on {\tt census} data ($|D|=32561$) with no privacy cost constraint:
        (a) shows one dimensional histogram queries where errors are correctly bounded by $\alpha=104$;
		(b) and (c) show the same conclusion for one dimensional prefix queries and two dimensional histogram queries, respectively.}\label{fig:}
\end{figure*}



\begin{figure*}[h]
	\centering
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/census_accuracy_1d_hist_icq}%
		\caption{ICQ 1-D Histogram Queries using LCM}
		\label{fig:census_hist_1d_icq_lcm}
	\end{subfigure}%
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/census_accuracy_1d_prefix_icq}%
		\caption{ICQ 1-D Histogram Queries using OM}
		\label{fig:census_hist_1d_icq_om}
	\end{subfigure}%
	\begin{subfigure}[h]{0.33\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/census_accuracy_1d_hist_tcq}%
		\caption{TCQ 1-D Histogram Queries}
		\label{fig:census_hist_1d_tcq}
	\end{subfigure}%
	\caption{Accuracy of ICQ and TCQ of fixed $(0.0032|D|, 0.0005)$-accuracy with no privacy cost constraint. (a) and (b) were set with predicate threshold to $2\alpha$ (typiclly the $\alpha$ is much smaller than $c$). Both can achieve perfect accuracy. In (c), top $k=3$ predicates were selected}\label{fig:}
\end{figure*}

\todo{vary alpha, measure accuracy}
}

\subsection{Privacy Cost}

\begin{figure}[h]
	\centering
	\begin{subfigure}[h]{0.45\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_wcq}%
		\caption{Privacy cost of mechanisms w.r.t WCQ types}
		\label{fig:cost_wcq}
	\end{subfigure}
	\begin{subfigure}[h]{0.45\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_wcq_a}%
		\caption{Privacy cost of mechanisms varying workload sizes}
		\label{fig:cost_wcq_a}
	\end{subfigure}%
	\caption{Privacy Cost for WCQ}\label{fig:cost_wcq_all}
\end{figure}

\begin{figure*}[h]
	\centering
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_icq}%
		\caption{Vary ICQ type}
		\label{fig:cost_icq}
	\end{subfigure}%
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_icq_a1}%
		\caption{Vary workload size}
		\label{fig:cost_icq_a1}
	\end{subfigure}%
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_icq_a2}%
		\caption{ICQ-MPM Vary Poking Step}
		\label{fig:cost_icq_a2}
	\end{subfigure}%
	\caption{Privacy Cost for ICQ}\label{fig:cost_icq_all}
\end{figure*}


\begin{figure*}[h]
	\centering
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_tcq}%
		\caption{Vary TCQ types}
		\label{fig:cost_tcq}
	\end{subfigure}%
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_tcq_a1}%
		\caption{Vary TCQ workload size}
		\label{fig:cost_tcq_a1}
	\end{subfigure}%
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_tcq_a2_lm}%
		\caption{TCQ-LM Vary K}
		\label{fig:cost_tcq_a2_lm}
	\end{subfigure}%
	\begin{subfigure}[h]{0.25\textwidth}%
		\includegraphics[width=\textwidth]{../../figure/experiments/cost_tcq_a2_tm}%
		\caption{TCQ-TM Vary K}
		\label{fig:cost_tcq_a2_lm}
	\end{subfigure}%
	\caption{Privacy Cost for TCQ}\label{fig:cost_tcq_all}
\end{figure*}
